Gear-up for the Action Replay: Leveraging Lensing for Enhanced Gravitational-Wave Early-Warning

Pre-merger gravitational-wave (GW) sky-localisation of binary neutron star (BNS) and neutron star black hole (NSBH) coalescence events, would enable telescopes to capture precursors and electromagnetic (EM) emissions around the time of the merger. We propose a novel astrophysical scenario that could provide early-warning times of hours to days before coalescence with sub-arcsecond localisation, provided that these events are gravitationally lensed. The key idea is that if the BNS/NSBH is lensed, then so must the host galaxy identified via the EM counterpart. From the angular separation of the lensed host galaxy images, as well as its redshift and the (foreground) lens redshift, we demonstrate that we can predict the time delays assuming a standard lens model. Encouraged by the non-trivial upper limits on the detection rates of lensed BNS/NSBH mergers that we estimate for upcoming observing runs of the LIGO-Virgo-Kagra and third generation networks, we assess the feasibility and benefits of our method. To that end, we study the effect of limited angular resolution of the telescopes on our ability to predict the time delays. We find that with an angular resolution of $0.05''$, we can predict time delays of $> 1$ day with $1\sigma$ error-bar of $\mathcal{O}$(hours) at best. We also construct realistic time delay distributions of detectable lensed BNSs/NSBHs to forecast the early-warning times we might expect in the observing scenarios we consider.

==> rates.tex <==
We estimate the rates of lensed BNS and NSBH that will become detectable both with the upcoming (O4-O5 observing runs of LIGO--Virgo--Kagra) and future detector network sensitivities (e.g. Voyager and 3G detectors).
We note that there is a considerable uncertainty on the estimation of the detection rate of lensed BNSs/NSBHs. This in large part stems from the fact that no lensed BNSs/NSBHs have been observed so far, and barely a handful of corresponding unlensed systems have been observed with GWs. Nevertheless, we follow standard prescriptions delineated in the literature (see Appendix~\ref{app:rate} for additional details) to estimate the rate of lensed BNS and NSBH. The results are tabulated in Table~\ref{tab:rate}.

\begin{table}
\centering
\begin{tabular}{|l|c|c|c|c|c} \hline
Obs. & Lensed BNS $[\mathrm{yr}^{-1}]$ & Lensed NSBH $[\mathrm{yr}^{-1}]$ \\\hline
O4 & $0 - 0.3$ & $0.001 - 0.2$ \\\hline 
O5 & $0.005 - 10$ & $0.02 - 3.4$ \\\hline
Voyager & $0.3 - 617$ & $0.7 - 179$ \\\hline
3G & $12 - 34822$ & $12 - 4279$ \\\hline
\end{tabular}
\caption{Rates of detectable lensed BNS and NSBH events, for various observing scenarios. Only galaxy lenses are considered, which is expected to be a good approximation given the relative rarity of clusters. See Appendix~\ref{app:rate} for additional details on the assumptions used to estimate the rates.}
\label{tab:rate}
\end{table}

Even though the rate estimates have uncertainties that span multiple orders of magnitude, they suggest that seeing a lensed BNS or NSBH in O4 is unlikely, although not abysmally small assuming the optimistic upper limit. Seeing such an event in O5 appears more likely relative to O4. Voyager seems to be the first observing scenario that is almost certainly to see a lensed BNS or NSBH, and the 3G scenario guarantees it.

That said, ultimately, the detection of lensed BNSs/NSBHs will follow Poisson statistics, and a Poisson fluctuation may enable observations of such events even in O4 or O5. Indeed, being ready for such an event, in case one should present itself, could have dramatic scientific payoffs due to the drastic enhancement of early-warning times. As a result, we are interested in estimating uncertainties on the time delay predictions arising from various systematics. In this work, we focus on the astrometric uncertainties when analysing the optical images of the lensed host galaxy.    


